Mellotron: Multispeaker expressive voice synthesis by conditioning on rhythm, pitch and global style tokens

Mellotron is a multispeaker voice synthesis model based on Tacotron 2 GST that can make a voice emote and sing without emotive or singing training data. By explicitly conditioning on rhythm and continuous pitch contours from an audio signal or music score, Mellotron is able to generate speech in a variety of styles ranging from read speech to expressive speech, from slow drawls to rap and from monotonous voice to singing voice. Unlike other methods, we train Mellotron using only read speech data without alignments between text and audio. We evaluate our models using the LJSpeech and LibriTTS datasets. We provide F0 Frame Errors and synthesized samples that include style transfer from other speakers, singers and styles not seen during training, procedural manipulation of rhythm and pitch and choir synthesis.

==> relatedwork.tex <==
%auto-ignore
Approaches to expressive speech synthesis with prosody transfer and style transfer with learned latent factors \cite{skerry2018towards,wang2018style} have several limitations. First, learning latent factors of interest implies having a speech dataset wherein the factors of interest exist. For example, singing voice synthesis would requires a singing voice dataset. Arguably, even in such cases, there are no guarantees that the learned latent factor contains the desired characteristics. In addition, 

%(rprenger) I don't think we need paragraph about Voice Conversion.  It's seen as a different problem, so no one is going to ask why you didn't include it.  If you want to say you borrowed tricks from VC then that should be one sentence later (if at all)
Approaches to expressive synthesis through Voice Conversion (VC) also have several limitations. There are voice conversion methods\cite{qian2019zero} that factorize the source signal into a content embedding and a speaker embedding. A common failure mode in this setup occurs when the content embedding has information about the speaker and vice-versa. Hence, this approach requires the cumbersome task of finding the perfect balance between model architecture, content and speaker embedding size and loss terms. Surprisingly, despite of the success of automatic speech recognition systems (ASR) and their minimal computational cost, most voice conversion approaches do not condition on text, thus requiring the content embedding to contain all text information. We circumvent such pronunciation issues by conditioning Mellotron on text as well.

Finally, expressive speech synthesis can be approached through Singing Voice Synthesis (SVS)



Furthermore, approaches that rely on pitch and rhythm obtained from a MIDI file to reconstruct a target audio implicitly learns the singer's interpretation of the musical score. In such approaches, we lose complete control over the output pitch and rhythm and rely on the model to interpret the MIDI rendering to synthesize the audio. Last, unlike Mellotron, these approaches do not learn any latent factors.

%What are the key components of my approach and results? Also include any specific limitations.

%(rprenger) This paragraph is great and should be in the abstract

